Replicable Parallel Branch and Bound Search

Combinatorial branch and bound searches are a common technique for solving global optimisation and decision problems. Their performance often depends on good search order heuristics, refined over decades of algorithms research. Parallel search necessarily deviates from the sequential search order, sometimes dramatically and unpredictably, e.g. by distributing work at random. This can disrupt effective search order heuristics and lead to unexpected and highly variable parallel performance. The variability makes it hard to reason about the parallel performance of combinatorial searches. This paper presents a generic parallel branch and bound skeleton, implemented in Haskell, with replicable parallel performance. The skeleton aims to preserve the search order heuristic by distributing work in an ordered fashion, closely following the sequential search order. We demonstrate the generality of the approach by applying the skeleton to 40 instances of three combinatorial problems: Maximum Clique, 0/1 Knapsack and Travelling Salesperson. The overheads of our Haskell skeleton are reasonable: giving slowdown factors of between 1.9 and 6.2 compared with a class-leading, dedicated, and highly optimised C++ Maximum Clique solver. We demonstrate scaling up to 200 cores of a Beowulf cluster, achieving speedups of 100x for several Maximum Clique instances. We demonstrate low variance of parallel performance across all instances of the three combinatorial problems and at all scales up to 200 cores, with median Relative Standard Deviation (RSD) below 2%. Parallel solvers that do not follow the sequential search order exhibit far higher variance, with median RSD exceeding 85% for Knapsack.

==> sections/formalKnapsack.tex <==
One of the main features of parallel skeletons is the ability to maintain a
clear separation between the parallelism coordination features and the actual
work which is performed. To show our is generic enough to handle
other branch-and-bound applications, while maintaining the search ordering
properties, we apply it to the 0/1 knapsack problem.

The knapsack problem is one of the classic optimisation problems. Given a
container of some finite size and a set items, each with some size and value,
which items should we add to the container to maximise profit? Knapsack
problems have important applications such as bin-packing and industrial
decision making processes. Some interesting applications of knapsack may be
found in \cite{salkin.dekluyver_knapsackSurvey:1975}.

Variants of the knapsack problem are possible which generally change the
constraints on item choice. For example allowing items to be chosen multiple
times, or fractional parts of items to be selected.
\cite{martello.toth_knapsack:1990} discusses many of these variants, including
0/1 knapsack.

We only consider the 0/1 knapsack problem which allows full items to be chosen
only once.

At each step a bound may be calculated using \emph{continuous relaxation} where,
instead of solving for $i \in \{0,1\}$ we instead solve fractional knapsack
problem where $i \in [0,1]$. As the greedy fractional approach is optimal this
provides an upper bound on the maximum potential value. Although it is possible
to compute an upper bound on the entire computation by considering the choices
at the top level\cite{martello.toth_upperBoundKnapsack}, we do not this here.
The benefit you gain from such a method is stopping the computation early should
you find the theoretical maximum.

\subsubsection{Formalising the 0/1 Knapsack problem}

We are now in a position to formalise the 0/1 knapsack problem using the BBM. As
a running example we use the knapsack instance given in~\cref{tab:exampleKP}.

\begin{table}
  \centering
  \begin{tabular}{l c c}
    \toprule
    \textbf{Capacity:} & \multicolumn{2}{l}{\textbf{16}} \\
    \textbf{Id} & \textbf{Profit} & \textbf{Weight} \\ 
    \midrule
    0 & 45 & 3 \\
    1 & 30 & 5 \\
    2 & 45 & 9 \\
    3 & 10 & 5 \\
    \bottomrule
    \end{tabular}
  \caption{Example knapsack problem}
  \label{tab:exampleKP}
\end{table}

As the problem input, we are given a fixed capacity \(C\) and a set of \(m\)
items \(I = \{i_1 \dots i_m\}\). For each item define \(p : I \to \mathbb{N}\)
and \(w : I \to \mathbb{N}\) to be projection functions for the profit and
weight of an item respectively.

%TODO-BA: Doesn't quite read right
If we consider the input item set as a vector of items, then the 0/1 knapsack
problem is equivalent to creating a new vector vector \(X\) where \(x_j \in
\{0,1\}\), corresponding to the binary choice for each item \(i_j\) in the input
vector.

With this notation we can formally write the 0/1 knapsack problem as:

\begin{equation}
  \textbf{max} \sum_{j=1}^{m} p(i_j)x_j \quad \textbf{where}\; \sum_{j=1}^{m} w(i_j)x_j \leq C
\end{equation}

\subsection{Formulation in BBM}

BBM makes use of finite words to represent tree branches. We extend the
profit and weight functions, \(p\) and \(w\), to those operating on words (\(p :
I^* \to \mathbb{N}\) and \$w : I\(^{\text{*}}\) \(\to\) \(\mathbb{N}\)) by
taking the sum across each component.

Using the example in~\cref{tab:exampleKP}, consider the word \(i_1i_3\).
\(p(i_1i_3) = p(i_1) + p(i_3) = 30 + 10 = 40\). We use the same function name for both
the individual and word versions of the profit and weight function where it is
clear from the context.

%TODO-BA: Where do I want to put this? Probably here since it's used later on.
For efficient computation of a bound we place an initially order the items in
ascending order with respect to the \emph{profit density ordering} given by:

\begin{equation}
\frac{p(i_1)}{w(i_1)} \geq \frac{p(i_2)}{w(i_2)} \dots \geq \frac{p(i_n)}{w(i_n)}\;; where\; i \in I
\end{equation}

For our example the items are already given in this ordering.

\subsubsection{Generator Function}

We define an unordered tree generator, \(g : I^* \to 2^I\), for the 0/1 knapsack
problem is as follows:

% TODO-BA: Rewrite this formulation. It can technically allow us to pick any
% choice we haven't chosen already?
\begin{equation}
g(i_1 \dots i_m) = \{ i_j \in I ~|~ i_m < i_j \land w(i_1 \dots i_m) \leq C \}
\end{equation}

That is, given any current set of items, we can simply choose any that we
haven't seen before so long as the capacity constraint is met.

To extend this to an ordered generator, we take the values items found using the
unordered generator and order them in ascending order using the profit density ordering. 

In our example we have the following:

%TODO-BA: Change to the root graph symbol (check with @PM)
\begin{align*}
g(empty)  &= \{i_0,i_1,i_2,i_3\} \\
g(i_0)    &= \{i_1,i_2,i_3\} \\
g(i_0i_1) &= \{i_4\}
\end{align*}

\subsubsection{Objective Function}

The overall goal is to maximise the total profit in the knapsack. Because of
this, the objective function, \(f : I^* \to \mathbb{N}\) is simply \emph{p}, the profit
function over words. The ordering on objective functions \(\sqsubseteq\) is
simply given by the the natural ordering \(\leq\).

\subsubsection{Pruning Predicate}

We define the pruning predicate, \(p : \mathbb{N} \times I^* \to \{0,1\}\) as:

\begin{equation}
  p(bnd,(i_1 \dots i_m)) = 
  \begin{cases}
    1 & \textbf{if}\; p(i_1 \dots i_m) + fractionalKnapsack(I_{>i_m}, C - w(i_1 \dots i_m)) \leq bnd \\
    0 & otherwise
  \end{cases}
\end{equation}

Where: \(I_{>m} = \{i_j \in I ~|~ i_j\; \text{after}\; i_m\; \text{in the
profit-density ordering}\}\) 

The fractionalKnapsack function greedily solves a knapsack problem in which
fractional items may be chosen. Thus function runs in linear time and provides
an optimal solution making it ideal as an upper bound.

In our example:

\begin{align*}
bnd(i_0) &= 45 + fractionalKnapsack(\{i_1,i_2,i_3\}, 16 - 3) \\
fractionalKnapsack(\{i_1,i_2,i_3\}, 13) &= 30 + \frac{8}{9}\times45 = 70
\end{align*}

In this case no pruning would happen as the upper bound (\(115\) beats the current best
of \(45\)

%TODO-BA should we do a full example at the end with images etcq?

